DOLMA: A Data Object Level Memory Disaggregation Framework for HPC Applications

Memory disaggregation is promising to scale memory capacity and improves utilization in HPC systems. However, the performance overhead of accessing remote memory poses a significant challenge, particularly for compute-intensive HPC applications where execution times are highly sensitive to data locality. In this work, we present DOLMA, a Data Object Level M emory dis Aggregation framework designed for HPC applications. DOLMA intelligently identifies and offloads data objects to remote memory, while providing quantitative analysis to decide a suitable local memory size. Furthermore, DOLMA leverages the predictable memory access patterns typical in HPC applications and enables remote memory prefetch via a dual-buffer design. By carefully balancing local and remote memory usage and maintaining multi-thread concurrency, DOLMA provides a flexible and efficient solution for leveraging disaggregated memory in HPC domains while minimally compromising application performance. Evaluating with eight HPC workloads and computational kernels, DOLMA limits performance degradation to less than 16% while reducing local memory usage by up to 63%, on average.

==> contents/draft.tex <==



% \textbf{Platform.}  All experiments are conducted on an RDMA-based disaggregated system, in which we set up two nodes: the local node primarily conducts computation-intensive workloads, and the remote one serves as a memory node. Each node has two 24-core Intel(R) Xeon(R) Gold 6240R CPUs @ 2.40GHz. Each node has 187GB memory capacity.
% \name limits local node capacity based on peak memory consumption of the application. 
% Both nodes are equiped with Mellanox ConnectX-6 HDR100/100GbE VPI Adapters, which offer 100 Gbps InfiniBand connectivity.

%\textcolor{red} {NVIDIA Mellanox ConnectX-6 VPI; 100Gb/s (HDR100; EDR IB and 100GbE); single-port QSFP56; PCIe3.0 x16 Adapter.}
%The two nodes are connected through an Infiniband switch. 


%We used two nodes connected to an Infiniband switch on the chameleon cloud~\cite{mambretti2015next}. The first node acts as a compute node running HPC applications, the second node provides remote memory. Each node has a 24-core Intel(R) Xeon(R) Gold 6240R CPU @ 2.40GHz. We set the RDMA registered memory on the compute node to different sizes based on the peak memory usage of different applications and registered memory on the memory node to 10GB. These nodes are equipped with Mellanox ConnectX6NIC  with a 50 Gbps Infiniband network. 

% We exclude the remaining two NPB workloads, EP and SP, from the evaluation. EP’s memory usage is trivial (only consuming 0.1 GB at its peak), making it not necessary for assessing remote memory, while SP exceeds the available memory capacity in our platform, causing an out-of-memory error.
% \textcolor{red}{Haoyu, I need a more detailed explanation here:}
% \textcolor{purple}{We exclude the remaining two NPB workloads, EP and SP, from our evaluation due to their unrepresentative or impractical memory behaviors in the context of our remote memory study.
% Specifically, EP demonstrates extremely low memory demands, peaking at only 0.1 GB, which is negligible and does not stress the memory system enough to meaningfully evaluate the impact of remote memory mechanisms. Including such a case would not yield insightful comparisons across memory configurations. SP has a very large memory footprint that exceeds the physical DRAM capacity of our evaluation platform, causing an out-of-memory error.}


% on five NAS Parallel Benchmark (NPB) workloads, \textcolor{red}{as well as ... } which are summarized in table~\ref{table:workloads}. The workloads are derived from computational fluid dynamics (CFD) applications and consist of kernels and pseudo-applications. Specifically, the five workloads include (1) CG - Conjugate Gradient, which involves irregular memory access and communication; (2) MG - Multi-Grid on a sequence of meshes, which requires both long- and short-distance communication and is memory intensive; (3) FT - discrete 3D fast Fourier Transform, which involves all-to-all communication; (4) BT - Block Tri-diagonal solver; (5) LU - Lower-Upper Gauss-Seidel solver and \textcolor{red}{(6) IS - Integer Sort. \textcolor{red}{EP and SP are not included. EP's memory consumption is too small, which is not suitable for memory Disaggregation.The memory consumption of the SP benchmark exceeded the memory limitations of the chameleon cloud machine.}
% } \textcolor{red}{(Add some discussions about why not using other three benchmarks?)}


% \textbf{Workloads.} We evaluate our performance on five NAS Parallel Benchmark (NPB) workloads, \textcolor{red}{as well as ... } which are summarized in table~\ref{table:workloads}. The workloads are derived from computational fluid dynamics (CFD) applications and consist of kernels and pseudo-applications. Specifically, the five workloads include (1) CG - Conjugate Gradient, which involves irregular memory access and communication; (2) MG - Multi-Grid on a sequence of meshes, which requires both long- and short-distance communication and is memory intensive; (3) FT - discrete 3D fast Fourier Transform, which involves all-to-all communication; (4) BT - Block Tri-diagonal solver; (5) LU - Lower-Upper Gauss-Seidel solver and \textcolor{red}{(6) IS - Integer Sort. \textcolor{red}{EP and SP are not included. EP's memory consumption is too small, which is not suitable for memory Disaggregation.The memory consumption of the SP benchmark exceeded the memory limitations of the chameleon cloud machine.}
% } \textcolor{red}{(Add some discussions about why not using other three benchmarks?)}

%We use NPB Benchmark to evaluate the performance of data-level memory disaggregation.In table.1, we list the attributes of different problems setting. The eight benchmarks mimic the computation and data movement in HPC applications. It has five kernels, IS, EP, CG, MG, FT and three pseudo applications, BT, SP, and LU. There benchmarks cover different memory access patterns. We list these features in the Table 1. 

%\textbf{Baseline.} We compare our method to the application's Oracle execution. In the application' oracle execution, it only uses local memory. 

% \textcolor{red}{I need the workload table here.}
